Linked Crunchbase: A Linked Data API and RDF Data Set About Innovative Companies

Crunchbase is an online platform collecting information about startups and technology companies, including attributes and relations of companies, people, and investments. Data contained in Crunchbase is, to a large extent, not available elsewhere, making Crunchbase to a unique data source. In this paper, we present how to bring Crunchbase to the Web of Data so that its data can be used in the machine-readable RDF format by anyone on the Web. First, we give insights into how we developed and hosted a Linked Data API for Crunchbase and how sameAs links to other data sources are integrated. Then, we present our method for crawling RDF data based on this API to build a custom Crunchbase RDF knowledge graph. We created an RDF data set with over 347 million triples, including 781k people, 659k organizations, and 343k investments. Our Crunchbase Linked Data API is available online at http://linked-crunchbase.org.

==> overview.tex <==
Our workflow to create the Linked Data API is shown in Fig.~\ref{fig:flowchart}.
We first set up a simple RDF API to harvest an initial RDF data set 
%(an "RDF Dump File") 
via crawling. 
We use the initial RDF data set to enrich our Linked Data API with \texttt{owl:sameAs} links to DBpedia.
The obtained links are then integrated into the API, so that the links are available when a URI of the wrapper is dereferenced.

%%% 1. RDF API: %%%
We have implemented the Linked Data API for CrunchBase.
The code of the wrapper is available on GitHub\footnote{See \url{https://github.com/aifb/linked-crunchbase}, requested on Feb 5, 2016.} under the MIT license, and we maintain an instance of the wrapper.\footnote{See \url{http://km.aifb.kit.edu/services/crunchbase/}, requested on June 28, 2016.} 
Additional information about the wrapper is made available at the entry page. 
%\todo[inline]{use "entry page" throughout when referring to that page - not homepage or such} 
The wrapper provides data in different formats via content negotiation, and enriches CrunchBase entities retrieved from the CrunchBase REST API with \texttt{owl:sameAs} links to DBpedia, which is a hub in the Linking Open Data cloud. Besides the CrunchBase Linked Data API implementation, we provide a description of the service and of the used schema (predefined by CrunchBase) as OWL file and as VoID file.
%%
%% old: The RDF API returns the corresponding data stored in the CrunchBase database, but wraps it in the form of RDF. In addition, we enrich the RDF with links to DBpedia entities, since DBpedia is a hub in the linked open data cloud and since we can thereby use methods which are designed for DBpedia, such as many text annotation tools.


%%% 2. RDF dump: %%%

For setting up a local CrunchBase RDF Knowledge Base for research on news monitoring \cite{Faerber2016}, we built a CrunchBase RDF data set with the help of the implemented CrunchBase Linked Data API. We thereby restricted ourselves to facts of organizations, people, products, and acquisitions, since entities of those types contain the facts which are -- in our minds -- the most important for our news monitoring task. We crawled in October 2015 and retrieved 7,373,480 unique entities. 
% counted via rdf:type
The crawled CrunchBase RDF data set can be reused by all researchers who want to extend existing Knowledge Bases with CrunchBase data or who want to analyze the RDF data set for their own purposes. %in a semantic way.
%
%\todo[inline]{Where is that data available? -- @M: Create Table at the end with links.}
%% TODO (cm): maybe mention research in startup scene
%
%Note, however, that the CrunchBase data is released under the Creative Commons Attribution-NonCommercial 4.0 International Public License.\footnote{See \url{https://creativecommons.org/licenses/by-nc/4.0/}, requested on Feb 4, 2016.} Any crawled CrunchBase RDF data set is therefore only to be used for non-commercial purposes. 
